Gradient Informed Proximal Policy Optimization

We introduce a novel policy learning method that integrates analytical gradients from differentiable environments with the Proximal Policy Optimization (PPO) algorithm. To incorporate analytical gradients into the PPO framework, we introduce the concept of an {\alpha}-policy that stands as a locally superior policy. By adaptively modifying the {\alpha} value, we can effectively manage the influence of analytical policy gradients during learning. To this end, we suggest metrics for assessing the variance and bias of analytical gradients, reducing dependence on these gradients when high variance or bias is detected. Our proposed approach outperforms baseline algorithms in various scenarios, such as function optimization, physics simulations, and traffic control environments. Our code can be found online: https://github.com/SonSang/gippo.

==> rebuttal.tex <==
\begin{figure}[h]
\centering

    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=0.32\textwidth]{figures/rebuttal/ant/result_learning_graph.pdf}
         \includegraphics[width=0.32\textwidth]{figures/rebuttal/ant/alpha_graph_0.5.pdf}
         \includegraphics[width=0.32\textwidth]{figures/rebuttal/ant/oorr_graph_0.5.pdf}
         \caption{Statistics of training in \textbf{Ant} environment when $\delta_{oorr} = 0.5$.}
    \end{subfigure}
    
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=0.32\textwidth]{figures/rebuttal/ant/rebuttal_learning_graph.pdf}
         \includegraphics[width=0.32\textwidth]{figures/rebuttal/ant/alpha_graph_1.0.pdf}
         \includegraphics[width=0.32\textwidth]{figures/rebuttal/ant/oorr_graph_1.0.pdf}
         \caption{Statistics of training in \textbf{Ant} environment when $\delta_{oorr} = 1.0$.}
    \end{subfigure}
    
\caption{\textbf{Learning graph, $\alpha$ graph, and out-of-range-ratio graph in Ant environment.} Since we use out-of-range-ratio for upper bounding $\alpha$ during runtime, even when the analytical gradients are more useful than PPO-based approach, we cannot fully utilize them. (a) When $\delta_{oorr} = 0.5$, we can observe that $\alpha$ gradually decreases to fulfill this constraint, and thus out-of-range-ratio stays around $0.5$. However, because of this, GI-PPO exhibits slower learning speed compared to the RP method, as shown in the left learning graph. (b) In contrast, when $\delta_{oorr} = 1.0$, which means that $\alpha$ is not constrained by out-of-range-ratio anymore, GI-PPO shows slightly better results than the RP method. Note that the $\alpha$ stabilizes around $0.05$, and out-of-range-ratio is near $1$, which means that $\alpha$ policy is far away from the original policy, and PPO does not contribute much to the policy update. This observation tells us that we can further improve our approach by finding a way to pay more attention on analytical gradients than PPO based approach when they are more promising. Exploring how to do it in a systematic way is one of our future research directions.}
\end{figure}

==> tex/1-2_teaser_ackley.tex <==
\begin{figure}[t]
\vspace*{-1.5em}
\centering
    \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/teaser_ackley/3d_trajectory_whole.png}
         \vspace*{-2.5em}
         \caption{Entire optimization trajectory}
         \label{}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/teaser_ackley/3d_trajectory_partial.png}
         \vspace*{-2.5em}
         \caption{Partial optimization trajectory near optimum}
         \label{fig:teaser-b}
    \end{subfigure}
\caption{Reward surface and optimization trajectories of policy learning methods on 1-dimensional Ackley's function. The height of the reward surface represents the expected return of the distribution defined by mean and variance. (a) At an early stage, PPO (green) and GI-PPO (blue) converge faster to the optimum, while the RP-gradient-based method (yellow) encounters difficulties. (b) GI-PPO combines an initial policy update towards the $\alpha$-policy (light blue) with a subsequent PPO-based update step, resulting in significantly faster convergence to the optimum compared to the baseline PPO. The $\alpha$-policy is defined using analytical gradients, considering variance and biasedness.}
\vspace{-1.25em}
\label{fig:teaser}
\end{figure}

==> tex/5-1_pace_car_results.tex <==
\begin{figure*}[t]
\centering
    \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/pacecar_2023_01_22/2x2_learning_graph.pdf}
         \caption{2-lane pace car}
         \label{fig:exp-pace-car-2-lane}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/pacecar_2023_01_22/3x3_learning_graph.pdf}
         \caption{3-lane pace car}
         \label{fig:exp-pace-car-3-lane}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/pacecar_2023_01_22/4x4_learning_graph.pdf}
         \caption{4-lane pace car}
         \label{fig:exp-pace-car-4-lane}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/pacecar_2023_01_22/10x4_learning_graph.pdf}
         \caption{10-lane pace car}
         \label{fig:exp-pace-car-10-lane}
    \end{subfigure}
    \vspace{-1em}
\caption{Experimental results on pace car problem for traffic control. Each experiment was done for a different number of lanes. (a), (b) In 2-lane and 3-lane cases, our method converges to better policy faster than other baseline algorithms, but SHAC still performs as well as ours. (c) In the 4-lane case, our method achieves the best performance in fewer time steps than other baseline algorithms, and PPO also succeeds in achieving good results faster than SHAC. (d) In the 10-lane case, our method converges to the best result much faster than all other methods.}
\vspace{-1.5em}
\label{fig:exp-pace-car}
\end{figure*}

==> tex/5-2-1_physics_ant_oorr.tex <==
\begin{figure*}[h]
\centering

    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=0.32\textwidth]{figures/rebuttal/ant/result_learning_graph.pdf}
         \includegraphics[width=0.32\textwidth]{figures/rebuttal/ant/alpha_graph_0.5.pdf}
         \includegraphics[width=0.32\textwidth]{figures/rebuttal/ant/oorr_graph_0.5.pdf}
         \caption{Statistics of training in \textbf{Ant} environment when $\delta_{oorr} = 0.5$.}
    \end{subfigure}
    
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=0.32\textwidth]{figures/rebuttal/ant/rebuttal_learning_graph.pdf}
         \includegraphics[width=0.32\textwidth]{figures/rebuttal/ant/alpha_graph_1.0.pdf}
         \includegraphics[width=0.32\textwidth]{figures/rebuttal/ant/oorr_graph_1.0.pdf}
         \caption{Statistics of training in \textbf{Ant} environment when $\delta_{oorr} = 1.0$.}
    \end{subfigure}
    
\caption{\textbf{Learning graph, $\alpha$ graph, and out-of-range-ratio graph in Ant environment.} Since we use out-of-range-ratio for upper bounding $\alpha$ during runtime, even when the analytical gradients are more useful than PPO-based approach, we cannot fully utilize them. (a) When $\delta_{oorr} = 0.5$, we can observe that $\alpha$ gradually decreases to fulfill this constraint, and thus out-of-range-ratio stays around $0.5$. However, because of this, GI-PPO exhibits slower learning speed compared to the RP method, as shown in the left learning graph. (b) In contrast, when $\delta_{oorr} = 1.0$, which means that $\alpha$ is not constrained by out-of-range-ratio anymore, GI-PPO shows slightly better results than the RP method. Note that the $\alpha$ stabilizes around $0.05$, and out-of-range-ratio is near $1$, which means that $\alpha$ policy is far away from the original policy, and PPO does not contribute much to the policy update. This observation tells us that we can further improve our approach by finding a way to pay more attention on analytical gradients than PPO based approach when they are more promising. Exploring how to do it in a systematic way is one of our future research directions.}
\end{figure*}

==> tex/5-3_function_optim_results_old_.tex <==
\begin{figure*}[t]
\centering
    \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/function_optim/dejong_64_learning_graph.pdf}
         \caption{De Jong's function (64)}
         \label{}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/function_optim/dejong_2048_learning_graph.pdf}
         \caption{De Jong's function (2048)}
         \label{}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/function_optim/ackley_64_learning_graph.pdf}
         \caption{Ackley's function (64)}
         \label{}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/function_optim/ackley_2048_learning_graph.pdf}
         \caption{Ackley's function (2048)}
         \label{fig:ackley-2048}
    \end{subfigure}
    %\vspace{-0.75em}
\caption{Experimental results for classical function optimization problems. The dimension of each problem is noted in ``( )''. 
}
\vspace{-1.5em}
\label{fig:exp-func-optim}
\end{figure*}

==> tex/5-4_mujoco_results.tex <==
\begin{figure}[t]
\centering
    \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mujoco_results/ppo/2e-1/learning_graph_ant.png}
         \caption{PPO, Ant ($\alpha=0.2$)}
         \label{}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mujoco_results/ppo/2e-1/learning_graph_swimmer.png}
         \caption{PPO, Swimmer ($\alpha=0.2$)}
         \label{}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mujoco_results/trpo/4e-1/learning_graph_ant.png}
         \caption{TRPO, Ant ($\alpha=0.4$)}
         \label{}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mujoco_results/trpo/2e-1/learning_graph_swimmer.png}
         \caption{TRPO, Swimmer ($\alpha=0.2$)}
         \label{}
    \end{subfigure}
    %\vspace{-0.75em}
\caption{Experimental results for Mujoco problems using the first approach. Note that our method achieves convergence to a better policy in less time with proper $\alpha$ size.}
\vspace{-2.5em}
\label{fig:exp-mujoco}
\end{figure}

==> tex/5-5_diff_physics_results.tex <==
\begin{figure*}[t]
\centering
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/physics/ant.pdf}
         \caption{Ant}
         \label{}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/physics/hopper.pdf}
         \caption{Hopper}
         \label{}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/physics/humanoid.pdf}
         \caption{Humanoid}
         \label{}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/physics/cheetah.pdf}
         \caption{Cheetah}
         \label{}
    \end{subfigure}
    \vspace{-1em}
\caption{Experimental results for differentiable physics control problems. We have noted the learning rate for the policy gradient of Equation~\ref{eq:pg-rl} together in the legend. (a), (b), (c) In Ant, Hopper, and Humanoid environments, our method shows generally better, or at least similar performance over all learning rates. (b) On the other hand, in Cheetah, our method achieves slightly worse results than SHAC for all learning rates. Please see Appendix~\ref{} for graphical renderings of these environments.}
\vspace{-1.0em}
\label{fig:exp-diff-phys}
\end{figure*}

==> tex/7-1_approach_1_results.tex <==
%%%%%%%%%%%%%%%%%% PPO

\begin{figure}[h!]
\centering
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/approach_1_mujoco_results/ppo/Ant.pdf}
         \caption{Ant}
         \label{}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/approach_1_mujoco_results/ppo/Swimmer.pdf}
         \caption{Swimmer}
         \label{}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/approach_1_mujoco_results/ppo/HalfCheetah.pdf}
         \caption{HalfCheetah}
         \label{}
    \end{subfigure}
    
    \vspace{-0.5em}
\caption{Experimental results for enhanced importance sampling approach. We tested our method on the Ant, Swimmer, and HalfCheetah MuJoCo environments. Note that we use PPO from Stable Baselines 3 as the base policy gradient method.}
\label{fig:exp-approach-1-mujoco-ppo}
\end{figure}

\vspace{-1em}

%%%%%%%%%%%%%%%%%%%%%% TRPO

\begin{figure}[h!]
\centering
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/approach_1_mujoco_results/trpo/Ant.pdf}
         \caption{Ant}
         \label{}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/approach_1_mujoco_results/trpo/Swimmer.pdf}
         \caption{Swimmer}
         \label{}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/approach_1_mujoco_results/trpo/HalfCheetah.pdf}
         \caption{HalfCheetah}
         \label{}
    \end{subfigure}
    
    \vspace{-0.5em}
\caption{Experimental results for enhanced importance sampling approach. We tested our method on the Ant, Swimmer, and HalfCheetah MuJoCo environments. Note that we use TRPO from Stable Baselines 3 as the base policy gradient method.}
\label{fig:exp-approach-1-mujoco-trpo}
\end{figure}

\vspace{-1em}

%%%%%%%%%%%%%%%% PPO, but using many actors

\begin{figure}[h!]
\centering
    \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/approach_1_physics_results/ant.pdf}
         \caption{Ant}
         \label{}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/approach_1_physics_results/cheetah.pdf}
         \caption{Cheetah}
         \label{}
    \end{subfigure}
    
    \vspace{-0.5em}
\caption{Experimental results for enhanced importance sampling approach. We tested our method on the Ant and Cheetah environments implemented in a differentiable physics simulator.}
\label{fig:exp-approach-1-physics}
\end{figure}


==> tex/7-2_hyperparameters.tex <==
\begin{table}[h!]
  \centering
  \label{tab:appendix-physics-hyperparams}
  \begin{tabular}{c c c c c}
  \toprule
  {\textbf{Hyperparameter}} & \textbf{PPO} & \textbf{SHAC} & \textbf{GradPPO}\\
  \midrule
  Actor Network Size & [64, 64] & [64, 64] & [64, 64] \\ 
  Critic Network Size & [64, 64] & [64, 64] & [64, 64] \\ 
  Horizon Length & 1 & 1 & 1 \\
  Number of Parallel Environments & 64 & 64 & 64 \\ 
  Actor Learning Rate ($PG_{RL}$) & Adaptive KL (0.008) & - & Adaptive KL (0.008) \\
  Actor Learning Rate ($PG_{AG}$) & - & 1e-3 & 1e-3 \\
  Critic Learning Rate & - & 1e-3 & 1e-3 \\
  Minibatch Size & 64 & - & 64 \\
  $\gamma$ & 0.99 & 0.99 & 0.99 \\
  $\tau$ & 0.95 & 0.95 & 0.95 \\
  
  \bottomrule
  \end{tabular}
  \caption{Experiment hyperparameters for function optimization problems in Figure~\ref{fig:exp-func-optim}.}
\end{table}

\begin{table}[h!]
  \centering
  \label{tab:appendix-physics-hyperparams}
  \begin{tabular}{c c c c c}
  \toprule
  {\textbf{Hyperparameter}} & \textbf{SHAC} & \textbf{GradPPO}\\
  \midrule
  Actor Network Size (Ant, Hopper) & [128, 64, 32] & [128, 64, 32] \\ 
  Actor Network Size (Cheetah) & [64, 64] & [64, 64] \\ 
  Actor Network Size (Humanoid) & [256, 128] & [256, 128] \\ 
  Critic Network Size (Ant, Hopper, Cheetah) & [64, 64] & [64, 64] \\
  Critic Network Size (Humanoid) & [128, 128] & [128, 128] \\ 
  Horizon Length & 32 & 32 \\
  Number of Parallel Environments (Ant, Cheetah, Humanoid) & 64 & 64 \\
  Number of Parallel Environments (Hopper) & 256 & 256 \\ 
  Actor Learning Rate ($PG_{RL}$) & - & Adaptive KL (Depends on Setting) \\
  Actor Learning Rate ($PG_{AG}$) & 2e-3 & 2e-3 \\
  Critic Learning Rate (Ant, Cheetah) & 2e-3 & 2e-3 \\
  Critic Learning Rate (Hopper) & 2e-4 & 2e-4 \\
  Critic Learning Rate (Humanoid) & 5e-4 & 5e-4 \\
  Minibatch Size (Ant, Cheetah, Humanoid) & - & 2048 \\
  Minibatch Size (Hopper) & - & 4096 \\
  $\gamma$ & 0.99 & 0.99 \\
  $\tau$ & 0.95 & 0.95 \\
  
  \bottomrule
  \end{tabular}
  \caption{Experiment hyperparameters for differentiable physics problems in Figure~\ref{fig:exp-diff-phys}. Note that the desired KL divergence was chosen from $1e-4, 5e-4, 1e-3, 5e-3$ as in the experiment description.}
\end{table}

\begin{table}[h!]
  \centering
  \label{tab:appendix-physics-hyperparams}
  \begin{tabular}{c c c c c}
  \toprule
  {\textbf{Hyperparameter}} & \textbf{PPO} & \textbf{SHAC} & \textbf{GradPPO}\\
  \midrule
  Actor Network Size & [64, 64] & [64, 64] & [64, 64] \\ 
  Critic Network Size & [64, 64] & [64, 64] & [64, 64] \\ 
  Horizon Length & 32 & 32 & 32 \\
  Number of Parallel Environments & 64 & 64 & 64 \\ 
  Actor Learning Rate ($PG_{RL}$) & Adaptive KL (0.008) & - & Adaptive KL (0.008) \\
  Actor Learning Rate ($PG_{AG}$) & - & 1e-3 & 1e-3 \\
  Critic Learning Rate & - & 1e-3 & 1e-3 \\
  Minibatch Size & 64 & 64 & 64 \\
  $\gamma$ & 0.99 & 0.99 & 0.99 \\
  $\tau$ & 0.95 & 0.95 & 0.95 \\
  
  \bottomrule
  \end{tabular}
  \caption{Experiment hyperparameters for pace car problems in Figure~\ref{fig:exp-pace-car}.}
\end{table}

==> tex/7-3_mujoco_examples.tex <==
\begin{figure*}[h!]
\centering
    \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mujoco_screenshots/mjc_ant.png}
         \caption{Ant}
         \label{}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mujoco_screenshots/mjc_hopper.png}
         \caption{Hopper}
         \label{}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mujoco_screenshots/mjc_humanoid.png}
         \caption{Humanoid}
         \label{}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mujoco_screenshots/mjc_half_cheetah.png}
         \caption{Half Cheetah}
         \label{fig:ackley-2048}
    \end{subfigure}
    %\vspace{-0.75em}
\caption{Mujoco environment visualizations.
}
\vspace{-1.5em}
\label{fig:appendix-mujoco-examples}
\end{figure*}

==> tex/legacy_approach.tex <==
\subsection{Perturbed Policy $\barpieps$ using Gradient}

Now we define a new policy $\widetilde{\pi}_{\epsilon}$ by perturbing our current policy $\pi$ using gradient information from a differentiable simulator as

\begin{equation}
\begin{aligned}
\label{eq:perturbed-policy}
    &\qquad \qquad \widetilde{\pi}_{\epsilon}(\widetilde{a} | s) = \sum_{a} \pi(a|s) \\
    &\qquad \text{ where } \widetilde{a} = f(a) = a + \epsilon \nabla_{a}Q_{\pi}(s, a) \\
    &\text{ and constant } |\epsilon| < \frac{1}{\max_{a}|\det(\gradQsecond|)}.
\end{aligned}    
\end{equation}

The constraint on $\epsilon$ is to make the function $f$ bijective (Appendix). Note that we can estimate the first order and second order gradients, $\gradQfirst$ and $\gradQsecond$, with trajectories ($\tau$) that start from the state $s$.
\begin{equation}
\begin{aligned}
    \gradQfirst = \mathbb{E}_{\tau \sim \pi} \left [ \sum_{t=0}^{\infty}\gamma^{t} \nabla_{a}r_{t} \right ], \\
    \gradQsecond = \mathbb{E}_{\tau \sim \pi} \left [ \sum_{t=0}^{\infty}\gamma^{t} \nabla_{a}^{2}r_{t} \right ].
\end{aligned}
\end{equation}

Conceptually, in this new policy $\widetilde{\pi}_{\epsilon}$, the probability density of a certain action $\widetilde{a}$ is same as the that of the action that could be ``optimized'' to $\widetilde{a}$ using a single step of gradient ascent or descent for optimizing the state-value function $Q$. However, $\widetilde{\pi}$ does not qualify to be a valid probability distribution, as its sum is not guaranteed to be 1.

\begin{equation}
\label{eq:perturbed-policy-is-not-distribution}
    \int_{a}\widetilde{\pi}_{\epsilon}(a|s)da = 1 + \epsilon\int_{a}\pi(a|s)\nabla_{a}^{2}Q_{\pi}(s, a)da.
\end{equation}

See Appendix for the proof. We can observe that $\widetilde{\pi}$ deviates from a valid probability distribution farther as $\epsilon$ increases. 

Therefore, we can define another policy $\barpieps$ by slightly changing the $\tilpieps$ with second order gradients. Then it becomes tightly coupled with the original policy $\pi$, and qualifies to be a valid distribution.

\vspace{1em}
\begin{proposition} 
\label{proposition:valid-perturbed-policy}
    Define $\barpieps$ as follows:
    \begin{align*}
        &\barpieps(\bar{a}|s) = \sum_{a} \frac{\pi(a|s)}{1 + \epsilon \det{(\gradQsecond)}} \\
        &\quad \text{ where } \bar{a} = a + \epsilon \nabla_{a}Q_{\pi}(s, a).
    \end{align*}
    
    Then, for any subset $[\bar{a}_{0}, \bar{a}_{1}]$ in the perturbed action space, following holds:
    \begin{align*}
        \int_{\bar{a}_0}^{\bar{a}_1} \barpieps (\bar{a}|s) d\bar{a} = \sum_{i}\int_{a_0}^{a_1} \pi(a|s) da.
    \end{align*}
    
\end{proposition}
\vspace{1em}
    

In fact, this new policy $\bar{\pi}_{\epsilon}$ turns out to have higher approximate expected return than the current policy $\pi$ if the $\epsilon$ value is sufficiently small positive value. That is, $\bar{\pi}_{\epsilon}$ exhibits locally better performance than $\pi$. On the contrary, if the $\epsilon$ is sufficiently small negative value, the new policy shows worse performance than $\pi$.

\vspace{1em}
\begin{theorem}
\label{theorem:locally-better-policy}
    If $|\epsilon| \ll 1$, 
    \begin{equation}
    \begin{aligned}
        L_{\pi}(\bar{\pi}_{\epsilon}) - \eta(\pi) = O(\epsilon) \text{ when } \epsilon > 0, \\
        \eta(\pi) - L_{\pi}(\bar{\pi}_{\epsilon}) = O(\epsilon) \text{ when } \epsilon < 0.
    \end{aligned}
    \end{equation}
    
\end{theorem}
\vspace{1em}

We provide the proofs for these claims at the Appendix. As described in Section~\ref{section:preliminaries},
TRPO and PPO aims at maximizing $L_\pi(\bar{\pi})$. Therefore, $L_{\pi}(\barpieps)$ with larger (positive) $\epsilon$ could be more desirable choice than that with lower $\epsilon$. However, as $\epsilon$ grows, the reliability of the estimation declines since our formulation is based on local approximation. Therefore, we can observe a trade off here.

To resolve the trade off and find the optimal $\epsilon$ that corresponds to the optimal policy nearby, we can reformulate the optimization problem suggested in the Equation~\ref{eq:original-optimization} as 
\begin{equation}
     \epsilon = \text{argmax}_{\epsilon} \left [ L_{\pi}(\bar{\pi}_{\epsilon}) - \frac{4\xi \gamma}{{(1 - \gamma)}^{2}}D^{max}(\pi, \bar{\pi}_{\epsilon}) \right ].
\end{equation}

 Note that the search space is now confined to one dimensional value, $\epsilon$. Therefore, it admits much simpler optimization process than the original problem, but could give worse result than that at the same time. 
 
 However, evaluating $\bar{\pi}_{\epsilon}$ in this reformulated problem is computationally infeasible. This is because for a single action $\bar{a}$, we have to find out every action $a$ that satisfies the condition in the Equation~\ref{eq:perturbed-policy} to find out $\barpieps(\bar{a})$.

Therefore, in the next section, we discuss how we can practically use $\barpieps$ to enhance the training.

\subsection{Practical Application of $\barpieps$}

Instead of using $\barpieps$ to find the optimal policy along it, we can use it in the importance sampling estimator used in approximating $L_{\pi}(\bar{\pi})$ with Monte Carlo simulation~\cite{schulman2015trust}. In practice, we can estimate $L_{\pi}(\bar{\pi})$ with any sampling function $q(a)$ as

\begin{equation}
    L_{\pi}(\bar{\pi}) = \mathbb{E}_{s\sim \pi, a\sim q} \left [ \frac{\bar{\pi}(a|s)}{q(a)} A_{\pi}(s, a) \right ].
\end{equation}

Theoretically, $L_{\pi}(\bar{\pi})$ does not depend on the choice of $q$. However, in practice, the training quality depends on it, because some actions are more important than the others in some states. If the $q$ function samples those actions better than another, it could accelerate the learning process and produce better policies.  

Here we use $\barpieps$ for $q$, because it samples relatively important actions better than the original policy $\pi$. 

